Partially Observable Contextual Bandits with Linear Payoffs

The standard contextual bandit framework assumes fully observable and actionable contexts. In this work, we consider a new bandit setting with partially observable, correlated contexts and linear payoffs, motivated by the applications in finance where decision making is based on market information that typically displays temporal correlation and is not fully observed. We make the following contributions marrying ideas from statistical signal processing with bandits: (i) We propose an algorithmic pipeline named EMKF-Bandit, which integrates system identification, filtering, and classic contextual bandit algorithms into an iterative method alternating between latent parameter estimation and decision making. (ii) We analyze EMKF-Bandit when we select Thompson sampling as the bandit algorithm and show that it incurs a sub-linear regret under conditions on filtering. (iii) We conduct numerical simulations that demonstrate the benefits and practical applicability of the proposed pipeline.

==> ImportantNote.tex <==
An interesting extension of the ICASSP work is contextual bandit with NO context observation.
We assume that the context evolves according to an unknown linear dynamical system and the reward is linear in the context.

The key here is that we exploit the fact that the reward in each bandit iteration provides a linear measurement of the context. Using results from the work \cite{tsiamis2022online} with the observation being the reward, we can get an estimate of reward $r_{a,k}$ for each arm $a$ before it is revealed, and follows Algorithm 1 of \cite{yang2021bandit} from the third line onwards. One gap is that Algorithm 1 of \cite{yang2021bandit} needs a measure of confidence width $s_{a,t}$. We need to think about how to get this if we skip context estimation and directly predict reward.
